Clustering What Matters: Optimal Approximation for Clustering with Outliers

Clustering with outliers is one of the most fundamental problems in Computer Science. Given a set $X$ of $n$ points and two integers $k$ and $m$, the clustering with outliers aims to exclude $m$ points from $X$ and partition the remaining points into $k$ clusters that minimizes a certain cost function. In this paper, we give a general approach for solving clustering with outliers, which results in a fixed-parameter tractable (FPT) algorithm in $k$ and $m$, that almost matches the approximation ratio for its outlier-free counterpart. As a corollary, we obtain FPT approximation algorithms with optimal approximation ratios for $k$-Median and $k$-Means with outliers in general metrics. We also exhibit more applications of our approach to other variants of the problem that impose additional constraints on the clustering, such as fairness or matroid constraints.

==> euclidean.tex <==
%!TEX root = mainpaper.tex

\section{Extensions} \label{sec:extensions}

\subsection*{$k$-Means with Outliers}
This is similar to \kmedwo, except that the cost function is the sum of \emph{squares} of distances of all except $m$ outlier points to a set of $k$ facilities. This generalizes the well-known \kmeans problem. Here, the main obstacle is that, the squares of distances do not satisfy triangle inequality, and thus it does not form a metric. However, they satisfy a \emph{relaxed} version of triangle inequality (i.e., $\d(p, q)^2 \le 2 (\d(p, r)^2 + \d(r, q)^2)$). This technicality makes the arguments tedious, nevertheless, we can follow the same approach as for \kmedwo, to obtain optimal FPT approximation schemes. Our technique implies an optimal $(1+8/e + \epsilon)$-approximation for \kmeanswo (using the result of \cite{DBLP:conf/icalp/Cohen-AddadG0LL19} as a black-box), improving upon polynomial-time $53.002$-approximation from \cite{KrishnaswamyLS18}, and $(9+\epsilon)$-approximation from \cite{GoyalJ020} in time FPT in $k, m$ and $\epsilon$.

In fact, using our technique, we can get improved approximation guarantees for \kzwo, where the cost function involves $z$-th power of distances, where $z \ge 1$ is fixed for a problem. Note that the cases $z = 1$ and $z= 2$ correspond to \kmedwo and \kmeanswo respectively. We give the details for \kzwo in the appendix.

\subsection*{Matroid Median with Outliers} A \emph{matroid} is a pair $\mathcal{M} = (F, \mathcal{S})$, where $F$ is a ground set, and $\mathcal{S}$ is a collection of subsets of $F$ with the following properties: (i) $\emptyset \in \mathcal{S}$, (ii) If $A \in \mathcal{S}$, then for every subset $B \subseteq A$, $B \in \mathcal{S}$, and (iii) For any $A, B \in \mathcal{S}$ with $|B| < |A|$, there exists an $b \in B \setminus A$ such that $B \cup \{b\} \in \mathcal{S}$. The rank of a matroid $\mathcal{M}$ is the size of the largest independent set in $\mathcal{S}$. Using the definition of matroid, it can be easily seen that all inclusion-wise maximal independent sets (called \emph{bases}) have the same size.

An instance of \matmedwo is given by $(X, F, \mathcal{M}, m)$, where $\mathcal{M} = (F, \mathcal{S})$ is a matroid with rank $k$ defined over a finite ground set $F$, and $X, F$ are sets of clients and facilities, belonging to a finite metric space $(\Gamma, \d)$. The objective is to find a set $C \subseteq F$ of facilities that minimizes $\deltam{m}(X, C)$, and $C \in \mathcal{S}$, i.e., $C$ is an independent set in the given matroid. Note that an explicit description of a matroid of rank $k$ may be as large as $n^k$. Therefore, we assume that we are given an efficient \emph{oracle access} to the matroid $\mathcal{M}$. That is, we are provided with an algorithm $\mathcal{A}$ that, given a candidate set $S \subseteq F$, returns in time $T(\mathcal{A})$ (which is assumed to be polynomial in $|F|$), returns whether $S \in \mathcal{I}$. 

We can adapt our approach to \matmedwo in a relatively straightforward manner. Recall that our algorithm needs to start with an instance of outlier-free problem (i.e., \matmed) that provides a lower bound on the optimal cost of the given instance. To this end, given an instance $\cI= (X, F, \mathcal{M} = (F, \mathcal{S}), m)$ of \matmedwo, we define an instance $\cI' = (X, F, \mathcal{M'}, 0)$ of Matroid Median with $0$ Outliers (i.e., Matroid Median), where $\mathcal{M}' = (F \cup X, \mathcal{S}')$ is defined as follows. $\mathcal{S}' = \{Y \cup C : Y \subseteq X \text{ with } |Y| \le m \text{ and } C \subseteq F \text{ with } C \in \mathcal{S}\}$. That is, each independent set of $\mathcal{M}'$ is obtained by taking the union of an independent set of facilities from $\mathcal{M}$, and a subset of $X$ of size at most $m$. It is straightforward to show that $\mathcal{M}'$ satisfies all three axioms mentioned above, and thus is a matroid over the ground set $F \cup X$. In particular, it is the direct sum of $\mathcal{M}$ and a uniform matroid $\mathcal{M}_m$ over $X$ of rank $m$ (i.e., where any subset of $X$ of size at most $m$ is independent). Note that using the oracle algorithm $\mathcal{A}$, we can simulate an oracle algorithm to test whether a candidate set $C \subseteq F \cup X$ is independent in $\mathcal{M}'$. Therefore, using a $(2+\epsilon)$-approximation for \matmed \cite{DBLP:conf/icalp/Cohen-AddadG0LL19} in time FPT in $k$ and $\epsilon$, we can find a set $A \subseteq F \cup X$ of size at most $k+m$ that we can use to construct a coreset. The details about enumeration are similar to that for \kmedwo, and are thus omitted.

\subsection*{Colorful $k$-Median} 

This is an orthogonal generalization of \kmedwo to ensure a certain notion of \emph{fairness} in the solution (see \cite{JiaSS20}). Suppose the set of points $X$ is partitioned into $\ell$ different colors $X_1 \uplus X_2 \uplus \ldots \uplus X_\ell$. We are also given the corresponding number of outliers $m_1, m_2, \ldots, m_\ell$. The goal is to find a set of at most facilities $C$ to minimize the connection cost of all except at most $m_t$ outliers from each color class $X_t$, i.e., we want to minimize the cost function: $\sum_{t = 1}^\ell \deltam{m_t}(X_t, C)$. This follows a generalizations of the well-known $k$-\textsc{Center} problem introduced in \cite{Bandyapadhyay0P19} and \cite{AneggAKZ20,JiaSS20} , called \textsc{Colorful $k$-Center}. Similar generalization of \textsc{Facility Location} has also been studied in \cite{chekuri2022algorithms}. 

Using our ideas, we can find an FPT approximation parameterized by $k$, $m = \sum_{t = 1}^\ell m_t$, and $\epsilon$. To this end, we sample sufficiently many points from each color class $X_t$ separately, and argue that it preserves the cost appropriately. The technical details follow the same outline as that for $k$-Median with $m$ Outliers. In particular, during the enumeration phase---just like that for \kmedwo---we obtain several instances of \kmed. That is, our algorithm is \emph{color-agnostic} after constructing the coreset. Thus, we obtain a tight $(1+2/e+\epsilon)$-approximation for this problem. This is the first non-trivial true approximation for this problem -- previous work \cite{GuptaMZ21} only gives a \emph{pseudo-approximation}, i.e., a solution with cost at most a constant times that of an optimal cost, but using slightly more than $k$ facilities. 

\subsection*{A Combination of Above Generalizations}

Our technique also works for a combination of the aforementioned generalizations that are orthogonal to each other. To consider an extreme example, consider \textsc{Colorful Matroid Median} with $\ell$ different color classes (a similar version for $k$-\textsc{Center} objective has been recently studied by \cite{AneggKZ22}), where we want to find a set of facilities that is independent in the given matroid, in order to minimize the sum of distances of all except $m_t$ outlier points for each color class $X_t$. By using a combination of the ideas mentioned above, one can get FPT approximations for such generalizations. 

